Active-Region Tilt Angles from White-Light Images and Magnetograms: The Role of Magnetic Tongues

The presence of elongations in active region (AR) polarities, called magnetic tongues, are mostly visible during their emergence phase. AR tilts have been measured thoroughly using long-term white-light (WL) databases, sometimes combined with magnetic field information. Since the influence of magnetic tongues on WL tilt measurements has not been taken into account before, we aim to investigate their role in tilt-angle values and to compare them with those derived from LOS magnetograms. We apply four methods to compute the tilt angle of generally bipolar ARs: one applies the k-means algorithm to WL data, a second one includes the magnetic field sign of the polarities to WL data, and a third one uses the magnetic flux-weighted center of each polarity. The tilt values computed in any of these ways are affected by the presence of magnetic tongues. Therefore, we apply the newly developed Core Field Fit Estimator (CoFFE) method to separate the magnetic flux in the tongues from that in the AR core. We compare the four computed tilt-angle values, as well as these with the ones reported in long-term WL databases. For ARs with low magnetic flux tongues the different methods report consistent tilt-angle values. But for ARs with high flux tongues there are noticeable discrepancies between all methods indicating that magnetic tongues affect differently WL and magnetic data. However, in general, CoFFE achieves a better estimation of the main bipole tilt because it removes both the effect of tongues as well as the emergence of secondary bipoles when it occurs in between the main bipole magnetic polarities.

==> tilt_wl_labels.tex <==


\sect{Introduction}
\sect{Data}
\sect{Method}
   \sect{Mod_WL}
   \sect{Mod_MAG}
   \sect{CoFFE}
\sect{Tilt_ARS}
   \sect{Weak_tongues}
   \sect{Strong_tongues}
   \sect{Bipolar}
   \sect{Multipolar}     
\sect{Rem}
   \sect{Rem_Method}
   \sect{Rem_Asymmetry}
   \sect{Rem_Distribution_cB}
\sect{Conclusions}
\sect{Variety_tongues} % appendix


 1 \fig{example}
 2 \fig{11027_tilt}
 3 \fig{10879_tilt}
 4 \fig{9574_tilt}
 5 \fig{9906_tilt}
 6 \fig{11007_tilt}
 7 \fig{9748_tilt}
A.1 \fig{8760_10268_tilt}


